Consecutive Knowledge Meta-Adaptation Learning for Unsupervised Medical Diagnosis

Deep learning-based Computer-Aided Diagnosis (CAD) has attracted appealing attention in academic researches and clinical applications. Nevertheless, the Convolutional Neural Networks (CNNs) diagnosis system heavily relies on the well-labeled lesion dataset, and the sensitivity to the variation of data distribution also restricts the potential application of CNNs in CAD. Unsupervised Domain Adaptation (UDA) methods are developed to solve the expensive annotation and domain gaps problem and have achieved remarkable success in medical image analysis. Yet existing UDA approaches only adapt knowledge learned from the source lesion domain to a single target lesion domain, which is against the clinical scenario: the new unlabeled target domains to be diagnosed always arrive in an online and continual manner. Moreover, the performance of existing approaches degrades dramatically on previously learned target lesion domains, due to the newly learned knowledge overwriting the previously learned knowledge (i.e., catastrophic forgetting). To deal with the above issues, we develop a meta-adaptation framework named Consecutive Lesion Knowledge Meta-Adaptation (CLKM), which mainly consists of Semantic Adaptation Phase (SAP) and Representation Adaptation Phase (RAP) to learn the diagnosis model in an online and continual manner. In the SAP, the semantic knowledge learned from the source lesion domain is transferred to consecutive target lesion domains. In the RAP, the feature-extractor is optimized to align the transferable representation knowledge across the source and multiple target lesion domains.

==> tables.tex <==
% \begin{table}[H]
%     \setlength{\abovecaptionskip}{0cm}
%     \setlength{\belowcaptionskip}{-0.5cm}
%     \captionsetup{font=normal}
%     \caption{Classification Accuracy(\%) when meta-testing sets are: \textbf{SON},\textbf{PH2}}
%     \small
%     \centering

%     \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}
%     { |l| c c c c c c >{\columncolor{lightgray!30}}c |>{\columncolor{lightgray!30}}c|}
%     \hline
    
%     \hline
%         Methods & HAM
%           & D7P & SON & MSK & UDA & PH2 & Avg. & $\Delta$ \\
%     \hline
%     SourceOnly & \textbf{72.3} & 51.7 & 79.5
%             & 60.1 & 59.3 & 81.7 & 67.4 & $\Uparrow  7.0$ \\
%     JAN \cite{long2017deep} & 64.1 & 55.7 & 93.2
%              & 64.1 & 59.9 & 83.3 & 70.1 & $\Uparrow 4.3$ \\
%     DAN~\cite{ganin2016domain} & 68.5 & 57.5 & 96.0
%             & 67.3 & 62.1 & 83.3 & 72.5 & $\Uparrow 1.9$ \\
%     CaCo~\cite{huang2022category}& & & & & & & & $\Uparrow$\\
%     SSRT~\cite{sun2022safe}& & & & & & & & $\Uparrow$\\
%     RIPU~\cite{xie2022towards}& & & & & & & & $\Uparrow$\\
%     CDA(mer) \cite{long2018conditional} & & & & & & & & $\Uparrow$\\
%     DAN(ewc) \cite{kirkpatrick2017overcoming} & 68.9 & 53.2 & 82.3
%             & 58.8 & 57.7 & 78.3 & 66.5 &$\Uparrow 7.9$ \\
%     \hline
%     \hline
%     CLKM(fe) & 67.0 & 54.8 & 87.6 & 55.3 & 50.0 & 73.3 & 64.7 &$\Uparrow 9.7$ \\
%     CLKM(dq) & 68.1 & 59.7 & 96.5 & 63.2 & 58.8 & 83.3 & 71.6 &$\Uparrow 2.8$ \\
%     CLKM(f\&d) & 68.3 & 58.1 & 94.4 & 66.9 & 59.3 & 83.3 & 71.5 &$\Uparrow 2.9$ \\
%     CLKM(full) & 67.1& \textbf{61.3} & \textbf{98.9} & \textbf{69.4} & \textbf{63.2} & \textbf{86.7} & \textbf{74.4} & -\\
%     \hline
    
%     \hline
%     \end{tabular}
%     \label{tab2}
% \end{table}

% \begin{table}[H]
%     \setlength{\abovecaptionskip}{0cm}
%     \setlength{\belowcaptionskip}{-0.5cm}
%     \captionsetup{font=normal}
%     \caption{Classification Accuracy(\%) when meta-testing sets are: \textbf{D7P},\textbf{SON}}
%     \small
%     \centering

%     \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}
%     { |l| c c c c c c >{\columncolor{lightgray!30}}c |>{\columncolor{lightgray!30}}c|}
%     \hline
    
%     \hline
%         Methods & HAM
%           & D7P & SON & MSK & UDA & PH2 & Avg. & $\Delta$ \\
%     \hline
%     SourceOnly & 65.9 & 43.4 & 63.2
%             & 47.6 & 47.3 & 75.0 & 57.1 & $\Uparrow  17.0$ \\
%     JAN \cite{long2017deep} & 66.4 & 60.1 & 93.2
%              & 64.5 & 61.5 & 83.3 & 71.5 & $\Uparrow 2.6$ \\
%     DAN \cite{ganin2016domain} & \textbf{68.9} & 54.1 & 70.2 & 63.5 & \textbf{64.8} & 80.0 & 66.9 & $\Uparrow 7.2$ \\
%     CaCo~\cite{huang2022category}& & & & & & & & $\Uparrow$\\
%     SSRT~\cite{sun2022safe}& & & & & & & & $\Uparrow$\\
%     RIPU~\cite{xie2022towards}& & & & & & & & $\Uparrow$\\
%     CDA(mer) \cite{long2018conditional} & & & & & & & & $\Uparrow$\\
%     DAN(ewc) \cite{kirkpatrick2017overcoming} & 66.0 & 48.1 & 68.7
%             & 51.7 & 51.1 & 73.3 & 59.8 &$\Uparrow 14.3$ \\
%     \hline
%     \hline
%     CLKM(fe) & 68.3 & 60.1 & 97.4 & 64.8 & 61.0 & 80.0 & 71.9 &$\Uparrow 2.2$ \\
%     CLKM(dq) & 68.8 & \textbf{61.5} & 92.3 & 64.2 & 59.3 & 83.3 & 71.6 &$\Uparrow 2.5$ \\
%     CLKM(f\&d) & 68.2 & 61.3 & 99.2 & 68.2 & 61.0 & 81.7 & 73.2 &$\Uparrow 0.9$ \\
%     CLKM(full) & 67.5 & 61.3 & \textbf{99.8} & \textbf{68.6} & 62.6 & \textbf{85.0} & \textbf{74.1} & -\\
%     \hline
    
%     \hline
%     \end{tabular}
%     \label{tab3}
% \end{table}

% \begin{table}[H]
%     \setlength{\abovecaptionskip}{0cm}
%     \setlength{\belowcaptionskip}{-0.5cm}
%     \captionsetup{font=normal}
%     \caption{Classification Accuracy(\%) when meta-testing sets are: \textbf{D7P},\textbf{MSK}}
%     \small
%     \centering

%     \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}
%     { |l| c c c c c c >{\columncolor{lightgray!30}}c |>{\columncolor{lightgray!30}}c|}
%     \hline
    
%     \hline
%         Methods & HAM
%           & D7P & SON & MSK & UDA & PH2 & Avg. & $\Delta$ \\
%     \hline
%     SourceOnly & 70.3 & 47.0 & 76.8
%             & 54.5 & 56.0 & 76.7 & 63.6 & $\Uparrow 10.4 $ \\
%     JAN \cite{long2017deep} & 68.5 & 54.6 & 
%             88.7 & 60.1 & 57.1 & 81.7 & 68.5 & $\Uparrow 5.5 $ \\
%     DAN~\cite{ganin2016domain} & \textbf{74.7} & 45.7 & 87.0
%             & 55.0 & 52.2 & 80.0 & 65.8 & $\Uparrow 8.2$ \\
%     CaCo~\cite{huang2022category}& & & & & & & & $\Uparrow$\\
%     SSRT~\cite{sun2022safe}& & & & & & & & $\Uparrow$\\
%     RIPU~\cite{xie2022towards}& & & & & & & & $\Uparrow$\\
%     CDA(mer) \cite{long2018conditional} & & & & & & & & $\Uparrow$\\
%     DAN(ewc) \cite{kirkpatrick2017overcoming} & 70.6 & 47.0 & 86.3
%             & 55.8 & 54.9 & 85.0 & 66.6 &$\Uparrow 7.4$ \\
%     \hline
%     \hline
%     CLKM(fe) & 67.4 & 60.3 & 97.5 & 65.1 & 58.8 & 80.0 & 71.5 &$\Uparrow 2.5$ \\
%     CLKM(dq) & 68.4 & 60.1 & 96.0 & 61.9 & 58.8 & 81.7 & 71.1 &$\Uparrow 2.9$ \\
%     CLKM(f\&d) & 67.7 & 59.2 & 98.7 & 64.9 & 59.3 & 83.3 & 72.2 &$\Uparrow 1.8$ \\
%     CLKM(full) & 67.8 & \textbf{60.4} & \textbf{99.6} & \textbf{67.3} & \textbf{62.1} & \textbf{86.7} & \textbf{74.0} & -\\
%     \hline
    
%     \hline
%     \end{tabular}
%     \label{tab4}
% \end{table}

% \begin{table}[H]
%     \setlength{\abovecaptionskip}{0cm}
%     \setlength{\belowcaptionskip}{-0.5cm}
%     \captionsetup{font=normal}
%     \caption{Classification Accuracy(\%) when meta-testing sets are: \textbf{D7P},\textbf{UDA}}
%     \small
%     \centering

%     \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}
%     { |l| c c c c c c >{\columncolor{lightgray!30}}c |>{\columncolor{lightgray!30}}c|}
%     \hline
    
%     \hline
%         Methods & HAM
%           & D7P & SON & MSK & UDA & PH2 & Avg. & $\Delta$ \\
%     \hline
%     SourceOnly & 70.0 & 53.2 & 76.6 
%             & 61.7 & 57.7 & 81.7 & 66.8 & $\Uparrow  6.6$ \\
%     JAN~\cite{long2017deep} & 69.9 & 55.5 & \textbf{97.7}
%              & 58.3 & 54.9 & 78.3 & 69.1 & $\Uparrow 4.3$ \\
%     DAN~\cite{ganin2016domain} & 70.5 & 41.7 & 93.1
%         & 47.3 & 53.3 & 70.0 & 62.7 & $\Uparrow 10.7$ \\
%     CaCo~\cite{huang2022category}& & & & & & & & $\Uparrow$\\
%     SSRT~\cite{sun2022safe}& & & & & & & & $\Uparrow$\\
%     RIPU~\cite{xie2022towards}& & & & & & & & $\Uparrow$\\
%     CDA(mer) \cite{long2018conditional} & & & & & & & & $\Uparrow$\\
%     DAN(ewc) \cite{kirkpatrick2017overcoming} & 71.2 & 49.2 & 86.1
%             & 55.0 & 54.9 & 81.7 & 66.4 &$\Uparrow 7.0$ \\
%     \hline
%     \hline
%     CLKM(fe) & \textbf{72.6} & 54.4 & 77.7 & 60.1 & 56.0 & 78.3 & 66.5 &$\Uparrow 6.9$ \\
%     CLKM(dq) & 66.5 & 56.1 & 88.8 & 52.6 & 49.5 & 80.0 & 65.6 &$\Uparrow 7.8$ \\
%     CLKM(f\&d) & 71.0 & 56.6 & 82.1 & 64.7 & 59.3 & 80.0 & 69.0 &$\Uparrow$ 4.4\\
%     CLKM(full) & 67.9 & \textbf{60.6} & 93.7 & \textbf{67.8} & \textbf{62.1} & \textbf{88.3} & \textbf{73.4} & -\\
%     \hline
    
%     \hline
%     \end{tabular}
%     \label{tab5}
% \end{table}


% \begin{table}[H]
%     \setlength{\abovecaptionskip}{0cm}
%     \setlength{\belowcaptionskip}{-0.5cm}
%     \captionsetup{font=normal}
%     \caption{Classification Accuracy(\%) when meta-testing sets are: \textbf{MSK},\textbf{PH2}}
%     \small
%     \centering

%     \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}
%     { |l| c c c c c c >{\columncolor{lightgray!30}}c |>{\columncolor{lightgray!30}}c|}
%     \hline
    
%     \hline
%         Methods & HAM
%           & D7P & SON & MSK & UDA & PH2 & Avg. & $\Delta$ \\
%     \hline
%     SourceOnly & 68.7 & 50.5 & 77.9
%             & 56.6 & 56.0 & 80.0 & 64.9 & $\Uparrow 8.5$ \\
%     JAN~\cite{long2017deep} & 68.5 & 55.9 & 89.3
%              & 63.9 & 57.7 & 80.0 & 69.2 & $\Uparrow 4.2$ \\
%     DAN~\cite{ganin2016domain} & \textbf{72.9} & 45.0 & 91.3
%             & 47.9 & 55.5 & 76.7 & 64.9 & $\Uparrow 8.5$ \\
%     CaCo~\cite{huang2022category}& & & & & & & & $\Uparrow$\\
%     SSRT~\cite{sun2022safe}& & & & & & & & $\Uparrow$\\
%     RIPU~\cite{xie2022towards}& & & & & & & & $\Uparrow$\\
%     CDA(mer) \cite{long2018conditional} & & & & & & & & $\Uparrow$\\
%     DAN(ewc) \cite{kirkpatrick2017overcoming} & 69.4 & 47.4 & \textbf{99.9}
%             & 55.2 & 54.9 & 73.3 & 66.7 &$\Uparrow 6.7$ \\
%     \hline
%     \hline
%     CLKM(fe) & 68.6 & 59.4 & 96.3 & \textbf{69.1} & 56.6 & 80.0 & 71.7 &$\Uparrow 1.7$ \\
%     CLKM(dq) & 63.6 & \textbf{61.5} & 86.9 & 59.5 & \textbf{61.0} & \textbf{91.7} & 70.7 &$\Uparrow 2.7$ \\
%     CLKM(f\&d) & 68.1 & 60.6 & 99.0 & 65.8 & 59.3 & 81.7 & 72.4 &$\Uparrow 1.0$ \\
%     CLKM(full) & 67.7 & 61.3 & 99.2& 66.2 & 59.3 & 86.7 & \textbf{73.4} & -\\
%     \hline
    
%     \hline
%     \end{tabular}
%     \label{tab6}
% \end{table}

% \begin{table}[H]
%     \setlength{\abovecaptionskip}{0cm}
%     \setlength{\belowcaptionskip}{-0.5cm}
%     \captionsetup{font=normal}
%     \caption{Classification Accuracy(\%) when meta-testing sets are: \textbf{UDA},\textbf{PH2}}
%     \small
%     \centering

%     \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}
%     { |l| c c c c c c >{\columncolor{lightgray!30}}c |>{\columncolor{lightgray!30}}c|}
%     \hline
    
%     \hline
%         Methods & HAM
%           & D7P & SON & MSK & UDA & PH2 & Avg. & $\Delta$ \\
%     \hline
%     SourceOnly & 68.4 & 47.2 & 61.0
%             & 52.0 & 53.9 & 80.0 & 60.4 & $\Uparrow 11.9$ \\
%     JAN \cite{long2017deep} & 65.6 & 46.6 &
%             81.5 & 48.8 & 49.5 & 66.7 & 59.8 & $\Uparrow 12.5$ \\
%     DAN~\cite{ganin2016domain} & \textbf{73.8} & 52.6 & 93.3& 61.2 & 56.6 & 81.7 & 69.9 & $\Uparrow 2.4$ \\
%     CaCo~\cite{huang2022category}& & & & & & & & $\Uparrow$\\
%     SSRT~\cite{sun2022safe}& & & & & & & & $\Uparrow$\\
%     RIPU~\cite{xie2022towards}& & & & & & & & $\Uparrow$\\
%     CDA(mer) \cite{long2018conditional} & & & & & & & & $\Uparrow$\\
%     DAN(ewc) \cite{kirkpatrick2017overcoming} & 71.1 & 54.8 & \textbf{99.0} 
%             & 58.2 & 61.0 & 83.3 &  71.2 &$\Uparrow 1.1$ \\
%     \hline
%     \hline
%     CLKM(fe) & 70.2 & 55.9 & 94.0 & 67.0 & 59.3 & 81.7 & 71.3 &$\Uparrow 1.0$ \\
%     CLKM(dq) & 67.5 & 60.1 & 94.5 & 64.0 & 59.9 & 81.7 & 71.3 &$\Uparrow 1.0$ \\
%     CLKM(f\&d) & 68.7 & 58.6 & 84.0 & \textbf{68.3} & 61.5 & \textbf{90.0} & 71.9 &$\Uparrow 0.4$ \\
%     CLKM(full) & 67.3 & \textbf{60.3} & 
%     92.5 & 67.4 & \textbf{61.5} & 85.0 & \textbf{72.3} & -\\
%     \hline
    
%     \hline
%     \end{tabular}
%     \label{tab7}
% \end{table}

